How Much Coffee Was Consumed During EMNLP 2019? Fermi Problems: A New Reasoning Challenge for AI

Many real-world problems require the combined application of multiple reasoning abilities employing suitable abstractions, commonsense knowledge, and creative synthesis of problem-solving strategies. To help advance AI systems towards such capabilities, we propose a new reasoning challenge, namely Fermi Problems (FPs), which are questions whose answers can only be approximately estimated because their precise computation is either impractical or impossible. For example, "How much would the sea level rise if all ice in the world melted?" FPs are commonly used in quizzes and interviews to bring out and evaluate the creative reasoning abilities of humans. To do the same for AI systems, we present two datasets: 1) A collection of 1k real-world FPs sourced from quizzes and olympiads; and 2) a bank of 10k synthetic FPs of intermediate complexity to serve as a sandbox for the harder real-world challenge. In addition to question answer pairs, the datasets contain detailed solutions in the form of an executable program and supporting facts, helping in supervision and evaluation of intermediate steps. We demonstrate that even extensively fine-tuned large scale language models perform poorly on these datasets, on average making estimates that are off by two orders of magnitude. Our contribution is thus the crystallization of several unsolved AI problems into a single, new challenge that we hope will spur further advances in building systems that can reason.

==> sections/discussion-UNUSED.tex <==
% \begin{figure*}[h!]
%     \centering
%     % \begin{subfigure}{.45\textwidth}
%     \begin{lstlisting}[frame=single]
%     Q0: How many litres of water does the school use each week?
    
%     Q1: What is the duration of the week in days?
%     Q2: What is the total water consumption by students in the school?
%     Q3: What is the individual water consumption of a student?
%     Q4: What is the total number of students in the school?
    
%     F1: There are 7 days in a week.
%     F2: An average student's water consumption per day amounts to 18 litres
%     F3: The total number of students in the school is 516
    
%     A1: 7
%     A2: 18 L
%     A3: 516
    
%     Q0 -> Mul (Q1, Q2)
%     Q1 -> A1 | F1
%     Q2 -> Mul (Q3, Q4)
%     Q3 -> A2 | F2
%     Q4 -> A3 | F3
%     \end{lstlisting}
%     % \end{subfigure}
%     % \hspace{10pt}
%     % \begin{subfigure}{.45\textwidth}
%     % \begin{lstlisting}[frame=single]
%     % Q0: How many baseballs fit in a schoolbus?
%     % Q1: What is the volume of a baseball?
%     % Q2: What is the volume of a schoolbus? 
%     % \end{lstlisting}
%     % \end{subfigure}
%     \caption{\ak{Placeholder for showing example failure cases modulo space constraints}}
%     \label{fig:real_example}
% \end{figure*}

\section{Discussion} 

In this section, we introspect on the proposed FP challenge and datasets while discussing limitations of our work and potential for future research in this direction. \ak{nascent stage}
\\ \\
\noindent \textbf{Limitations and Future Work.} 
In this dataset, we only consider FPs that have a number as the final answer. 
However, there can be binary yes/no FPs (\eg Does the empire state building weigh more than a thousand blue whales?) and comparison FPs (\eg Which is longer? Distance from Earth to Moon or all the spaghetti on Earth arranged in a straight line?). 
However, our datasets do not consider them -- these are interesting extensions of the FPs considered in this work and test for the same set of reasoning skils. 

Further, this work only highlights the reasoning skill of abstraction and proposes FPs as an ideal candidate for evaluating it. 
While solving FPs is an appropriate downstream task, constructing datasets tailored to learn such abstractions would not only help solve FPs but also significantly improve the reasoning capabilities of AI systems. 
\\ \\
\noindent\textbf{Potential Sources of Bias.} Mining real questions instead of asking humans (e.g., via crowd-sourcing platforms) reduces the possibility of linguistic biases in the dataset. 
\ac{Are there biases introduced by the web-pages that we mined these from?} \ak{The dataset has a high US-centric bias, both in cultural context and vocabulary \etc}

==> sections/rel_work-old-v1.tex <==
% \begin{table*}[t!]
% \centering
% {\small
% \begin{tabular}{p{0.3\textwidth} p{0.45\textwidth} p{0.1\textwidth}}
% % \begin{tabularx}{\textwidth}{ccccc}
% \hline
% \textbf{Dataset} & \textbf{Reasoning type} & \textbf{Requires knowledge retrieval?} \\
% \hline
% \texttt{DROP} \cite{dua-etal-2019-drop} & counting, addition, sorting, etc. &  \xmark \\
% \texttt{HOTPOTQA} \cite{yang-etal-2018-hotpotqa} &  comparison, ..., etc. & \checkmark \\
% \texttt{QAngaroo} \cite{10.1162/tacl_a_00021} & ? & \xmark \\
% \texttt{StrategyQA} \cite{geva2021strategyqa} & comparison \pc{SQA has more than this!} & \checkmark \\
% \texttt{ComplexWebQuestions} \cite{talmor-berant-2018-web} & superlatives, comparatives, union, intersection, addition & \checkmark \\
% \texttt{MultiRCcorpus} \cite{khashabi-etal-2018-looking} & implied counts, sentiments, relationships & \xmark \\ 
% \texttt{QASC} \cite{Khot_Clark_Guerquin_Jansen_Sabharwal_2020}  & common-sense reasoning & \checkmark \\ 
% \texttt{OpenBookQA} \cite{Mihaylov2018CanAS} &  world-knowledge, common-sense reasoning & \checkmark \\ 
% \hline 
% \dset & world-knowledge, common-sense, mathematical reasoning & \checkmark \\ 
% \hline 
% \end{tabular}
% }
% \caption{Comparison of \dset~with existing datasets. \dset~uniquely contains `complex' questions that typically require mathematical reasoning in order to answer. \ac{TODO: Rethink column-headings, verify all entries, add missing datasets.}
% }
% \label{tab:dataset-comparison}
% \end{table*}


\section{Related Work}

% Fermi Problems (FPs) are a open-domain reasoning problems whose solution requires the combined application of various reasoning skills including employing suitable abstraction, commonsense knowledge based reasoning and the ability to decompose problems into simpler solvable chunks. 

%%%%%%%%%%%%
\subsection{Comparison with Existing Datasets}

Table~\ref{tab:dataset-comparison} provides a summary of related existing datasets.

\paragraph{Mathematical Reasoning.} 
There has been considerable interest in recent times to study the limits of performing mathematical computation and reasoning using neural networks \cite{saxton2019analysing, lample2019deep, hendrycks2021measuring, nogueira2021investigating}.
These works range from testing AI on simple computations that occur in high-school level algebra word problems to more complex ones like solving differential equations. 
While this is a crucial skill for AI, the proposed Fermi Problem Challenge tests for more fundamental reasoning skills (\eg spatial abstraction, commonsense reasoning, \etc) while transferring the burden of computing an answer to a ``calculator''. 
For instance, consider the question -- ``How many baseballs fit in a schoolbus?''. 
We are interested in systems that are able to infer that the solution requires the dividing the volume of the school bus and the volume of a baseball. 
The mathematical operation is quite simple and this part can easily be off-loaded to a calculator.
However, unlike the above mathematical reasoning papers, FPs test for the ability of an AI system to estimate the required quantities (\ie volumes of a baseball and a schoolbus) --  a complex reasoning task that tests for a completely different set of skills as opposed the above works. 

Additionally, it is important to highlight that Fermi Problem Olympiads require humans to do these calculations and, additionally, test for the ability to perform quick computations -- for example, approximating that a day has $25$ hours instead of $24$ makes calculations like $25\times60$ simpler for humans! 
However, computers don't have this limitation and therefore, we believe that testing for these skills as part of the FP challenge is less meaningful. 
% ,an ability to estimate quantities, and multi-hop mathematical reasoning -- each of which have so far remained independent areas of study. 

% \paragraph{Multi-hop inference in Reading Comprehension.} 
\paragraph{Multi-hop Reasoning.} 
Recently, there have been several large datasets that are aimed at answering questions via multi-hop inference. 
% DROP: A Reading Comprehension Benchmark Requiring Discrete Reasoning Over Paragraphs 
The \texttt{DROP} \cite{dua-etal-2019-drop} reading comprehension benchmark, which focuses on paragraph understanding, requires discrete reasoning (counting, sorting, addition, etc.) over entities provided in a passage. 
% Looking Beyond the Surface: A Challenge Set for Reading Comprehension over Multiple Sentences
Similarly, \texttt{MultiRCcorpus} \cite{khashabi-etal-2018-looking} contains questions with possibly multiple correct answers that need to be inferred from multiple sentences. 
% Smaller multi-hop reading comprehension datasets are the FraCaS test suite, (Weston et al., 2016), TriviaQA () .
% Constructing Datasets for Multi-hop Reading Comprehension Across Documents 
% HotpotQA: A Dataset for Diverse, Explainable Multi-hop Question Answering 
On the other hand, questions in the QAngaroo datasets \cite{10.1162/tacl_a_00021} and \texttt{HOTPOTQA} \cite{yang-etal-2018-hotpotqa} require aggregating information spread across multiple documents. 
%  reasoning over multiple sup- porting documents to answer; (2) the ques- tions are diverse and not constrained to any pre-existing knowledge bases or knowledge schemas; (3) we provide sentence-level sup- porting facts required for reasoning, allowing QA systems to reason with strong supervision and explain the predictions; (4) we offer a new type of factoid comparison questions to test QA systems’ ability to extract relevant facts and perform necessary comparison. 
% The Web as a Knowledge-Base for Answering Complex Questions -- \texttt{ComplexWebQuestions} 
\citet{talmor-berant-2018-web} leverage WebQuestionsSP \cite{yih-etal-2016-value}, an existing dataset of simple questions and the Freebase KB \cite{10.1145/1376616.1376746} to generate complex questions that are compositions of simpler questions. 
% constructed using existing knowledge bases (KBs). As a result, these datasets are constrained by the schema of the KBs they use, and therefore the diversity of questions and an- swers is inherently limited
% OpenBookQA -- requires using a given scientific fact, and an (unknown) additional fact to answer the question. 
% QASC: A Dataset for Question Answering via Sentence Composition
\texttt{OpenBookQA} \cite{Mihaylov2018CanAS} and \texttt{QASC} \cite{Khot_Clark_Guerquin_Jansen_Sabharwal_2020} contain multiple-choice questions that require composing multiple scientific facts. 
The questions in all these datasets are a function of a context -- a paragraph, documents or KB entries. However, Fermi problems are open-response questions that are characterized by unbiased associations -- entities that may never have been considered together in  the same context, e.g., `How many toothpicks will fill up an Olympic swimming pool?'. 
% These datasets are aimed at the reading comprehension task, i.e., answering questions based on some relevant information. 

% Many recent question-answering datasets also focus on multi-hop reasoning. 
% Did Aristotle Use a Laptop? A Question Answering Benchmark with Implicit Reasoning Strategies 
\texttt{StrategyQA} \cite{geva2021strategyqa} is a recent dataset with interesting questions such as, `Did Aristotle Use a Laptop?'. Fermi problems are similar in that they can also be solved by many different strategic decompositions. However, while \texttt{StrategyQA} questions only require comparison operations with a boolean result, Fermi problems require complex mathematical reasoning. 

\paragraph{Commonsense Reasoning.} \ak{Discuss -- CommonsenseQA \cite{talmor-etal-2019-commonsenseqa} \etc.}

\paragraph{Grounded Reasoning.} \ak{Cite various efforts in vision + language + reasoning -- potential future direction as FPs require imagination \etc for spatial abstraction, a common theme in FPs.}


%%%%%%%%%%%%
\subsection{Modeling Techniques}

\noindent \textbf{Numeracy in Large-scale Language Models.} Large-scale language models trained on web-scale data not surprisingly contain various common numerical facts -- \eg number of days in a year, distance from earth to moon, number of hairs on a human head, etc. 
Recent works \cite{spithourakis2018numeracy, berg-kirkpatrick-spokoyny-2020-empirical, zhang-etal-2020-language-embeddings} not only test for numerical facts captured by these models but also propose and analyse different encoding strategies for numbers.
We leverage this by using pre-trained checkpoints \as{`checkpoints' is an implementational notion; I would use something more abstract, such as pre-trained LMs (to refer to T5) or pre-trained LMs fine-tuned on XYZ (for fine-tuned models)} of such language models -- specifically, the T5 pre-trained model proposed by \citet{raffel2019exploring}.

Further, we see that a question-answering model fine-tuned from this checkpoint \ak{\cite{maqaw} cite maqaw paper} performs only slightly better than predicting a constant value for all FPs -- we present more details in \cref{sec:exp}.
However, tightly integrating such systems to provide estimates for intermediate steps in the FP solution is an interesting future direction for research.



% \cite{suhr-etal-2019-corpus} A Corpus for Reasoning about Natural Language Grounded in Photographs
%  Table \ref{tab:datasets} provides a summary of the similarities and differences between the different QA datasets. 

% \paragraph{Reasoning.} 
% In contrast to the relatively simple reasoning required in the above question answering tasks, the task of solving math problems requires more complex mathematical reasoning. 
% \ac{Todo.} 
% AI2 dataset -- Solving math word problems by verb categorization -- \cite{hosseini-etal-2014-learning}, and automatically solving algebra word problems \cite{kushman-etal-2014-learning}. 
% The algebraic word problems dataset with intermediate steps (rationales) by \citet{ling-etal-2017-program}, and its extension, the \texttt{MathQA} by \cite{amini-etal-2019-mathqa},  ....
% AllArith dataset -- \cite{DBLP:journals/tacl/RoyR18} -- Mapping to Declarative Knowledge for Word Problem Solving. 
% Koncel-Kedziorski et al., 2015; Clark et al., 2016

% \paragraph{Compositional reasoning.}
% CLEVR (Johnson), NLVR (Suhr et al. 2017), NLVR2 (Suhr et al., 2019) -- compositional reasoning in grounded language. 

